Breaking the Sample Size Barrier in Model-Based Reinforcement Learning with a Generative Model

This paper is concerned with the sample efficiency of reinforcement learning, assuming access to a generative model (or simulator). We first consider $\gamma$-discounted infinite-horizon Markov decision processes (MDPs) with state space $\mathcal{S}$ and action space $\mathcal{A}$. Despite a number of prior works tackling this problem, a complete picture of the trade-offs between sample complexity and statistical accuracy is yet to be determined. In particular, all prior results suffer from a severe sample size barrier, in the sense that their claimed statistical guarantees hold only when the sample size exceeds at least $\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^2}$. The current paper overcomes this barrier by certifying the minimax optimality of two algorithms -- a perturbed model-based algorithm and a conservative model-based algorithm -- as soon as the sample size exceeds the order of $\frac{|\mathcal{S}||\mathcal{A}|}{1-\gamma}$ (modulo some log factor). Moving beyond infinite-horizon MDPs, we further study time-inhomogeneous finite-horizon MDPs, and prove that a plain model-based planning algorithm suffices to achieve minimax-optimal sample complexity given any target accuracy level. To the best of our knowledge, this work delivers the first minimax-optimal guarantees that accommodate the entire range of sample sizes (beyond which finding a meaningful policy is information theoretically infeasible).

==> No-perturbation-section.tex <==
\section{New part}


Denote $\widehat{\bm Q}^{\star}$ as the optimal action value function to the empirical MDP $\widehat{\mathcal{M}}=(\cS,\cA, \widehat{\bm P}, \bm r, \gamma)$ 
with empirical probability transition kernel $\widehat{\bm P}$. 
Let $\widehat{\bm Q}$ represent an $\omega$-optimal action value function of the $\widehat{\mathcal{M}}$, namely, 
\begin{align}
		\forall (s,a) \in \mathcal{S} \times \mathcal{A}, \qquad 
		|\widehat{Q}(s,a) - \widehat{Q}^{\star}(s,a)|  \leq  \omega.
\end{align}
Given any pre-specified order of $\mathcal{A}$, a constant $\xi$ to be specified, 
generate a random variable $\zeta \sim \mathsf{Unif}(0,\xi)$ 
and define policy $\widehat{\pi}$ as 
\begin{align}
\label{eq:policy-Q}
\forall s \in \mathcal{S}, \qquad \widehat{\pi}(s) \defn \min \{a \in \mathcal{A}: \widehat{Q}(s,a) > \widehat{V}(s) - \zeta\},
\end{align}
where $\widehat{V}(s) \defn \max_a \widehat{Q}(s,a)$.



Following this choice of policy, the corresponding action value function and value function satisfy the following property. 
\begin{theorem}[Model-based planning]
\label{thm:sample-no-perturbation}
	There exist some universal constants $c_0,c_1>0$ such that for any $\delta > 0$ and any $0<\varepsilon \leq \frac{1}{1-\gamma}$, the policy $\widehat{\pi}$ defined in \eqref{eq:policy-Q} obeys
	%
	\begin{align*}
		\forall (s,a) \in \mathcal{S} \times \mathcal{A}, \qquad 
		V^{\widehat{\pi}}(s)  \geq  V^\star(s) - \varepsilon
		\qquad \text{and} \qquad
		 Q^{\widehat{\pi}}(s,a)  \geq  Q^\star(s,a)  - \gamma \varepsilon 
	\end{align*}
	%
	with probability at least $1-\delta$, provided that $\omega \leq c_1(1-\gamma)\varepsilon$, $\xi = c_1(1-\gamma)\varepsilon$ and that 
	the sample size per state-action pair exceeds 
	%
	\begin{align}
		N \geq \frac{c_{0}\log\big(\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)\varepsilon 
		\delta}\big)}{(1-\gamma)^{3}\varepsilon^{2}}  . 
	\end{align}
	%
\end{theorem}
\noindent The proof of this result is given in Section~\ref{sec:decouple-no-perturb}.

